Machine Learning for Wireless Link Quality Estimation: A Survey

Since the emergence of wireless communication networks, a plethora of research papers focus their attention on the quality aspects of wireless links. The analysis of the rich body of existing literature on link quality estimation using models developed from data traces indicates that the techniques used for modeling link quality estimation are becoming increasingly sophisticated. A number of recent estimators leverage machine learning (ML) techniques that require a sophisticated design and development process, each of which has a great potential to significantly affect the overall model performance. In this paper, we provide a comprehensive survey on link quality estimators developed from empirical data and then focus on the subset that use ML algorithms. We analyze ML-based link quality estimation (LQE) models from two perspectives using performance data. Firstly, we focus on how they address quality requirements that are important from the perspective of the applications they serve. Secondly, we analyze how they approach the standard design steps commonly used in the ML community. Having analyzed the scientific body of the survey, we review existing open source datasets suitable for LQE research. Finally, we round up our survey with the lessons learned and design guidelines for ML-based LQE development and dataset collection.

==> Bio/bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{gregor}}]{Gregor Cerar}	
	received his Master's degree in telecommunications from the Faculty of Electrical Engineering, University of Ljubljana, in 2016. He is currently pursuing a Ph.D. degree with the Jo\v{z}ef Stefan International Postgraduate School. He is also a research assistant with the Department of Communication Systems, Jo\v{z}ef Stefan Institute. His main research interests are in IoT, wireless networking of constrained devices, and machine learning applications in IoT.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{halil}}]{Halil Yetgin}	
	received the B.Eng. degree in computer engineering from Selcuk University, Turkey, in 2008, the M.Sc. degree in wireless communications
	from the University of Southampton, U.K., in 2010, and the Ph.D. degree in wireless communications with the Next Generation Wireless Research Group, 
	University of Southampton in 2015. He is an Assistant Professor with the Department of Electrical and Electronics Engineering, 
	Bitlis Eren University, Turkey and a research fellow at the Department of Communication Systems of Jo{\v z}ef Stefan Institute, Ljubljana, Slovenia. His research interests include the development of intelligent communication systems, energy efficient cross-layer design and resource allocation of the future wireless communication networks. He was a recipient of the full scholarship granted by the Republic of Turkey, Ministry of National Education.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mihael}}]{Mihael Mohor{\v c}i{\v c}}
	received the B.Sc., M.Sc., and Ph.D. degrees in electrical engineering from the University of Ljubljana, Ljubljana, in 1994, 1998, and 2002, respectively, 
	and the M.Phil. degree in electrical engineering from the University of Bradford, Bradford, U.K., in 1998. 
	He is currently the Head of the Department of Communication Systems and a Scientific Counsellor with the Jo{\v z}ef Stefan Institute, 
	and an Associate Professor with the Jo{\v z}ef Stefan International Postgraduate School. He has authored or co-authored over 200 refereed journal and conference papers, 
	co-authored three books and contributed to nine book chapters. His research interests include the development and performance evaluation of network protocols and 
	architectures for mobile and wireless communication systems, and resource management in terrestrial, stratospheric, and satellite networks. 
	His recent research interest is focused on cognitive radio networks, smart applications of wireless sensor networks, dynamic composition of communication services, 
	and wireless experimental testbeds. He participated in many EC co-funded research projects since 1996 and is currently involved in H2020 projects Fed4FIRE+, SAAM, RESILOC and BD4OPEM.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.25in,clip,keepaspectratio]{carolina}}]{Carolina Fortuna}
	received her B.Sc. in 2006, Ph.D. in 2013 and was a postdoctoral research associate at IBCN, Ghent University, 2014-2015. 
	Currently she is research fellow at the Department of Communication Systems, Jo{\v z}ef Stefan Institute and an assistant at the Jo{\v z}ef Stefan International Postgraduate School. 
	Her research is interdisciplinary, focusing on data and knowledge driven modelling of communication and sensor systems. She has participated in H2020, FP7 and FP6 projects. 
	In H2020 WiSHFUL she was the technical leader of the project on behalf of UGhent/iMinds while in FP7 CREW she was the technical leader of the JSI team. 
	She co-authored over 50 peer-reviewed publications, was TPC member at IEEE ICC 2011, 2012, 2013, 2014, 2016, ESWC 2012, 
	IEEE Globecom 2011, 2016, VTC 2010, 2016, IEEE WCNC 2009.
\end{IEEEbiography}
